Unsafe at Any Copy: Name Collisions from Mixing Case Sensitivities

File name confusion attacks, such as malicious symbolic links and file squatting, have long been studied as sources of security vulnerabilities. However, a recently emerged type, i.e., case-sensitivity-induced name collisions, has not been scrutinized. These collisions are introduced by differences in name resolution under case-sensitive and case-insensitive file systems or directories. A prominent example is the recent Git vulnerability (CVE-2021-21300) which can lead to code execution on a victim client when it clones a maliciously crafted repository onto a case-insensitive file system. With trends including ext4 adding support for per-directory case-insensitivity and the broad deployment of the Windows Subsystem for Linux, the prerequisites for such vulnerabilities are increasingly likely to exist even in a single system. In this paper, we make a first effort to investigate how and where the lack of any uniform approach to handling name collisions leads to a diffusion of responsibility and resultant vulnerabilities. Interestingly, we demonstrate the existence of a range of novel security challenges arising from name collisions and their inconsistent handling by low-level utilities and applications. Specifically, our experiments show that utilities handle many name collision scenarios unsafely, leaving the responsibility to applications whose developers are unfortunately not yet aware of the threats. We examine three case studies as a first step towards systematically understanding the emerging type of name collision vulnerability.

==> ExploitOverview.tex <==
\section{The exploitability of name collisions }




\subsection{Exploitable Cases}
\label{subsec:exploit}

\trent{Collisions not always exploitable.  Exploit is possible if collision leads to one principal gaining previously unauthorized permissions.  We identify three ways that a principal may gain permissions as the result of a collision.  I think we can make the cases simpler and more fundamental (e.g., DAC instead of Biba).  Can you detail an example that would cause each case for files?  F3 is close.  Can you make  more concrete as an example?}
\trent{What are the conditions that a principal needs to cause each type of collision?}
Due to collisions, we will always end up with fewer number of total objects (i.e. file/directories) when copying objects to a case insensitive filesystem. If collisions occur among objects of different privilege levels, then the following security concerns arise:

\paragraph{File Collisions}

\begin{enumerate}[label=F\arabic*.]
  \item End up with the low integrity version.\\
  \textbf{Problem:} A HIGH integrity process uses this file.

For example, consider collision between files `foo' (perm=755) and `FOO' (perm=777). The copy utility only creates `FOO'. Since anyone can update the `FOO', we cannot certify the integrity of the file.

  \item End up with a more permissive version.\\
  \textbf{Problem:} A SECRET process writes to this file.

For example, consider collision between files `foo' (perm=700) and `FOO' (perm=755). The copy utility only creates `FOO'. When a privileged process writes to `FOO', others can also read it.

  \item Leak data over a special file like named pipe or device file.\\
  \textbf{Problem:} Contents of a SECRET file are dumped into a more permissive named pipe.
\end{enumerate}

Certain copy utilities silently replace colliding files. If the colliding files have different integrity or privileges levels, then it can result in F1 or F2 respectively.

At times the copy utilities do not handle special files correctly. If a special file collides with a regular file, then the copy utility writes the contents of the regular file to the special file (say a named pipe). This becomes a security concern (F3) when the special and regular files have different privilege levels.

\paragraph{Directory Collisions}

\begin{enumerate}[label=D\arabic*.]
  \item End up with low integrity files in a HIGH integrity directory (i.e. merging HIGH and LOW integrity directories).\\
  \textbf{Problem:} A HIGH integrity process uses LOW integrity files form the merged directory.

  \item End up with SECRET files in a public directory (i.e. merging SECRET and PUBLIC directories).\\
  \textbf{Problem:} SECRET files are publicly accessible.
  % ex. httpd case: adding .htaccess file to data/
\end{enumerate}

Copy utilities can silently merge directories with colliding names. If the colliding directories have different integrity or privileges levels, then it can result in D1 or D2 respectively.

\subsection{Consequences}

Collisions (both case and encoding) can lead to the following consequences:

\begin{enumerate}
\item Data Loss
    \begin{description}
    \item[metadata] lost xattrs: results in missing MAC labels
    \item[contents] lost files; ex. unsupported file types like symlinks
    \end{description}
\item Data Leakage
    \begin{description}
    \item[type confusion] write data to different file type (ex. pipe, device etc.)
    \end{description}
\item Data Corruption
    \begin{description}
    \item[metadata] incorrect properties associated w/ wrong files (ex. apply more permissive permissions on files)
    \item[contents] ex. file data truncated due to collision
    \item[name] makefile replaced w/ Makefile -- can result in malicious builds. \todo{More concrete example scenario where this is bad.}
    \end{description}
\end{enumerate}


\subsection{A survey of likely vectors and selected case studies}
\JS{EXPAND:  In the following sections we survey the vulnerabilities observed in one class of likely victims for name collision exploits, namely, system utilities for copying files, and then discuss a series of case studies }

==> Makefile <==
# Programs
LATEX = pdflatex
BIBTEX = bibtex

# All template files
TEMPLATES = template*/*

main.pdf: *.tex *.bib figures/* $(TEMPLATES)
	$(LATEX) main
	-$(BIBTEX) main
	$(LATEX) main
	$(LATEX) main

clean:
	$(RM) \
		*.bbl *.blg *.aux \
		*.log *.synctex.gz *.out \
		main.pdf


==> SecurityImplications.tex <==
\section{Threat Model}
\label{sec:threat}
 
This paper assumes a threat model typical of those in file system
attack research.  We assume that any file system resource that an
adversary has permission to modify could be modified maliciously
(i.e., is an {\em adversary-controlled} resource).  If an adversary is authorized to modify a resource, an
adversary can modify that resource's data and metadata,
including the resource's filename.  We assume that an adversary will
attempt to create name collisions by either varying case or encodings
in filenames.  We assume that the adversary knows the victim
file system well enough to identify targets of collisions to which the
victim has the permissions to modify.
 
We assume that when a victim performs an operation that may modify the
file system (e.g., moves or copies the resource) under the attack conditions described in \autoref{subsec:model}, there is the potential for a name collision attack.
We assume that the victims may perform any file system operations that
the file system permissions authorize.  We assume that the adversary
does not know whether the victim employs any further defenses in
accessing the target resource (e.g., preventing use of symbolic
links).

Name collision attacks may be used to exploit the secrecy and integrity of the target resource.  First, a name collision in a copy operation enables the adversary to overwrite or replace the target resource's data and metadata with the source resource's data and metadata, compromising the integrity of the target resource.  Second, an adversary can exploit name collisions to gain unauthorized access to the victim’s secret data. An
adversary may gain read access to victim resources by changing the permission metadata of unauthorized resources through a collision as described above and/or exploiting the
ability to modify a sensitive resource that governs the operation of the victim program (e.g., configuration file) to cause a data leak.
%\trent{Note that squatting with a pipe is a traditional file squat attack.}
We also note that name collisions can lead to denial-of-service attacks. Any defenses that are employed may be flawed, such that a command that leads to a name collision may result in the system utility used to perform the operation to crash or hang unexpectedly.

Several widely relied-upon programs are at-risk to name collision attacks, including utilities 
for moving files within a file system (e.g., {\tt cp}, {\tt mv}, {\tt rsync}, etc.) or for processing repositories/archives (e.g., {\tt tar}, {\tt zip}, {\tt git}, etc.).  While these utilities
have a variety of configuration options, they appear to have fewer options related to preventing name confusion attacks (i.e., not just name collisions) than the variants of {\tt open} (e.g., {\tt openat}).  For example, {\tt cp} only provides controls over whether to follow symbolic links or not, but does not provide the features of {\tt openat} or {\tt openat2}, which provide control over how a pathname is resolved.  Thus, a question is whether such utilities provide sufficient controls to limit attacks from name collisions and whether applications and system scripts that invoke these utilities do so in ways that are at-risk to name collisions.




\begin{comment}

Under this model, the following operations can lead to collisions:
\begin{description}
\item[move/copy objects] This involves moving, or copying files from a source to a target. Standard system utilities such as cp, tar, rsync, etc. are generally used for this operation. Refer to \autoref{sec:tooling} for collisions leading to security issues.

% We can defend against this by enforcing case-consistency.

\item[use existing objects] Applications that assume a case-sensitive file system can unexpectedly run into collisions. For example, say that an application wants to create two files {\tt foo} and {\tt FOO} (in that order). If collisions are not handled, then the file {\tt foo} will be overwritten with the contents of {\tt FOO}.

\end{description}
 
% attacks
% secrecy and integrity
 
\subsection{Attack Surface}
% --------------------------

Name collisions expand the ways that alias and squat vulnerabilities may be exploited, increasing the attack surface that programs must defend to prevent exploitation.  Researchers have shown that alias and squat attacks are only possible if a program accesses files (i.e., system resources accessed using the file system) using a directory to which an adversary has write permission.  Name collisions expand this attack surface in two ways.  First, name collisions may cause more file names to possibly be directed to adversary-chosen files, making it more difficult for victims to determine whether they face attacks.  As described above, file names need to be canonicalized before the program can be sure that they do not collide with an existing file.  Second, programs have check for name collisions when they copy (or move, etc.) an adversary-controlled file into any target directory, as name collisions in the target directory may enable exploits.  In this case, adversaries do not even require write access to the target directory to launch exploits.


%Collisions provide additional attack vectors for adversaries to lure victims to modify their own file systems in ways that grant adversaries unauthorized access.
% lure victim to use name in filesys mod operation
%   git example
%First, adversaries can create malicious resources with filenames that collide with the filenames of unauthorized resources in case-insensitive file systems.
%Then, when a victim uses such adversary-named resources in operations that modify a case-insensitive file system (e.g., move or copy) where the target of the operation is unauthorized to the adversary, then a collision vulnerability may be exploited.
It is this expanded attack surface that enables exploitation of the \git\ vulnerability for the adversary to obtain arbitrary code execution.  First, the malicious repository contains a symbolic link 'a' that collides with the directory 'A' when both are copied by \git\ into the target directory.  Thus, when \git\ attempts to clone 'A/post-checkout' it instead creates the file '.git/hooks/post-checkout'.  Second, because \git\ is performing these copies, it has the permissions to create scenario in which the file squat using 'a' is possible in the target directory.  
% use dir of accessible to other 
%   mod other resource 
As a result, name collisions enable additional ways for adversaries to provide names to lure victims to access unauthorized resources on their behalf, a form of a {\em confused deputy attack}~\cite{confused-deputy}.  This includes the vector for providing malicious names remotely through repositories and/or archives.

Name collisions can be exploited to compromise the secrecy and/or the
integrity of victim data.  If an adversary can induce the victim to
move or copy an adversary-controlled resource to a file system location
that is unauthorized to the adversary, the adversary may be able to write an
unauthorized resource by selecting a name that collides with the name
of that unauthorized resource.  An adversary may use such collisions to modify the contents and/or metadata of the unauthorized resource.  In addition, an
adversary can exploit name collisions to gain unauthorized access to
the victim's secret data.  An adversary may gain read access to victim
resources by changing the permission metadata of the unauthorized
resources through a collision as described above and/or exploiting the ability to modify a sensitive resource (e.g., configuration file) to cause a data leak. 
% dos

We also note that name collisions can also lead to denial-of-service attacks.  A problem is that any defenses that may be employed may be flawed, such that a command that leads to a name collision may result in the system utility used to perform the operation to hang unexpectedly.  
 
% relationship to link/squat
 
Name collisions may be exploited in combination with the more
traditional aliasing and squat attacks.  In the \git\ vulnerability
example, a name collision is created with an alias (i.e., a symbolic
link) to overwrite victim resources.  Similarly, an adversary may use
a file squatting attack to place resources in locations that may
induce name collisions.  For example, an adversary may create a pipe
file at the location to which a victim may move or copy a file with
secret data to enable the adversary to redirect those secrets to the
adversary via the pipe.  While this attack is similar to a traditional
file squat, the adversary relies on a name collision (i.e., multiple
names that map to the same file resource) to implement the attack.
When file system resources are moved or copied, leading to a name
collision, \textit{defenses to prevent such attacks are inconsistent}, as we
see in Section~\cite{sec:uils}.  \trent{NOTE: File squat defenses on
  file creation will prevent this attack, but not necessarily on
  move/copy.}

There are three attack vectors where bad things can happen. These are:

% Clarify what the access is
\begin{enumerate}[label=A\arabic*.]
	\item Attacker has access to \emph{old file system}.\\
	\textbf{Example.} In the case of \git, the attacker can craft a repository.

	\item Attacker has access to \emph{new file system}.\\
	\textbf{Example.} In the case of Samba-based backups, the attacker can access the restore location.

	\item The \emph{new file system} already contain files/directories which get merged on copying files/directories.\\
	\textbf{Example.} When archives such as tar, zip, etc. are expanded, the attacker can gain access access by carefully crafting filenames and thereby forcing a name collision. Some utilities silently ignore existing files while others silently replace existing files.

When the existing files are \emph{silently ignored}, then this results in a successful squat since the permissions are under adversary control.
\end{enumerate}

\iffalse
\subsection{Limitations of Current Defenses}
\label{subsec:limits}

%\trent{Move/copy vs open/create - above?}
%\trent{Goal: assess current defenses and attack surface}
%\trent{Expanded use of mixed case sensitivity in systems}
%\trent{system, utility, application}

% no broadly accepted system defense - even for aliases
% programmer defenses - no symlinks and exclusive create
% openat - 

Preventing name confusion attacks in general requires programmers to choose the appropriate system API/commands configured with the appropriate flags to block attacks while allowing desired functionality for their programs.  These API/command configurations can be quite complex, so a research question we explore in this paper is whether they enable protection against name collision attacks as well, and if so under what conditions.

Ideally, operating systems would prevent name confusion attacks, including name collision attacks, systematically in file system operations.  Unfortunately, researchers have found that it is not possible to provide a purely system defense that prevents name confusion (e.g., aliasing via TOCTTOU attacks) attacks without possibly incurring false positives~\cite{cai09oakland}.  While researchers have also explored defenses that utilize some program knowledge~\cite{jigsaw14usenix} (e.g., from program analysis), these defenses may still incur some false positives due to interactions between programs.  As a result, the task currently falls on the programmer to prevent name confusion attacks of all kinds.

For this work, we consider APIs/commands to access/create a single file (e.g., {\tt open}) and to move/copy a file to another part of the file system (e.g., {\tt cp}).  First, the {\tt open} system call has been extended to restrict link following (e.g., {\tt O\_NOFOLLOW flag}) to prevent some name confusion attacks.  In addition, new variants of {\tt open}, such as {\tt openat} and {\tt openat2}, have been proposed.  {\tt openat} is designed to prevent TOCTTOU attacks specifically by decomposing the traditional file opening operating into two steps.  {\tt openat2} has various flags to control {\em how} a file name is resolved to a file resource.  None of these calls explicitly address name confusion.  

Second, commands for moving files within a file system (e.g., {\tt cp}, {\tt mv}, {\tt rsync}, etc.) or from a repository/archive to a file system (e.g., {\tt tar}, {\tt zip}, {\tt git}, etc.) have variety of configuration options. However, they appear to have fewer options related to preventing name confusion attacks than the variants of {\tt open}.  For example, {\tt cp} only provides controls over whether to follow symbolic links or not, but does not provide the features of {\tt openat} or {\tt openat2}.  However, such commands may employ some of these APIs internally to limit attacks.  Unfortunately, a programmer has little insight into what is permitted.
\end{comment}


%\todo{should explain clone?}

%%%%%
%% Bit bucket
%%%%%




\begin{comment}
At present, there are no system defenses for detecting and/or preventing collisions in file system operations.  Current defenses aim to help programmers avoid vulnerabilities due to aliasing, but these defenses have only an indirect impact on collisions.

Current defenses aim to enable programmers to control their program's use of  aliases, especially symbolic links.  There is no accepted system defense that ensures that all uses of symbolic links are safe relative to a security property, and it has been conjectured that no such general property exists~\cite{cai09oakland}.  As a result, systems provide APIs for programmers to decide how to handle symbolic links.  Several file system APIs include flags to avoid using symbolic links entirely (e.g., {\tt O\_NOFOLLOW flag} for the {\tt open} system call), but in many cases programmers want to be able to use symbolic links.  More advanced commands for file allow programmers to manage {\em how} files are open, including the impact of symbolic links.  For example, the {\tt openat} system call enables the user to open a directory first to validate its legitimacy before opening the remaining path.
\fi

File system operations allow collisions as long as the victim has the file system permissions to perform the operations caused by the collision.  file system permissions allowed \git\ to create an exploitable collision because \git\ owns the directory created from 'A', which allows \git\ to perform the replacement caused by the collision from 'a'.  While the victim may employ restrictions on file system operations (e.g., via flags or specialized APIs) to prevent exploitation of collisions, such as preventing the use of symbolic links, victims often do not look for such problems in file systems that they create.  For example, \git\ erroneously assumed that the files it created were safe for subsequent use in building the cloned file system.  Further, due to the complexity of encodings, it is difficult to determine in advance if a collision may occur, as this depends on how the target file system interprets names.  As a result, programmer errors caused by collisions will be common.
\end{comment}


\begin{comment}
as we see below, name collisions are much more complex to detect because collisions may be caused by encodings as well as case insensitivity.  \todo{Can we run experiments on the number of encodings that may lead to collisions for filenames in practice?}  While we have long known the importance of filtering input when constructing file paths (e.g., ".." attacks), collisions present a significantly more extensive challenge.  \todo{Are there cases of link traversal or file squatting that we have to look out for here that we do not for aliasing?  Besides encodings?}
\end{comment}

\iffalse
\todo{TJ: I think we can eliminate all the text below.}
\todo{Types of attacks: squat, link traversal, input for names, TOCTTOU.  How do they work for name collisions?  Do not assume reader knows how these work at all.}
Developer induced bugs such as missing checks, unsanitized inputs, etc. lead to vulnerabilities in programs. The problems become more profound when applications get their inputs from untrusted sources.

Applications that use file names sourced from untrusted inputs can be victims of name confusion. Problems related to links have been well studied. However, issues arising from collisions (case/encoding) don't have many papers.

We argue that this is because collisions generally manifest themselves under cross file system use. Some example apps: git, tar, unzip, etc.

gist:

- apps not designed for cross-platform use. We mainly want to study cross file-system use.
- the ones that do have too many edge cases
- apps that rely on untrusted input for file names can be victims of name confusion. Here, adversary can file squat in the source directory.
  * direct access: ex. cp, rsync
  * via serialization format: ex. git, tar (the format is additional attack vector)
- apps trying to reason about name resolution can be imprecise: ex. assumes icase
- USP: we can detect these from syscall API

testing:

- apps that make assumptions about file systems being case sensitive can suffer from NC. For testing:
  * expects multiple resources (i.e. expects open() to returns a different resource)
  * expects unique resource (expects open() to return an existing resource) -- uses O\_EXCL
- example apps:
  * copy between source and target FS
  * is cross platform: works on multiple OS leading and hence can be exposed to collision attacks

ways to tackle this:

- black box testing with inputs (file names) and test outputs
- static analysis of programs
- monitor and hook into syscall interface

%Investigate the recent Git vulnerability (CVE-2021-21300). One of the issues is the cross FS use of Git across different OSes. We believe that apps are not unit tested with same rigor across file systems. We’re trying to identify issues that stem from peculiar/unique name resolution properties of different file systems. For example, case-sensitive vs. case-insensitive file systems. We have identified certain properties and scenarios that present unique challenges for developers. Further we believe that the POSIX API can be limiting since it doesn’t expose such peculiar properties of the underlying file system. However, case sensitivity is a system level property and developers should not have to worry about it.

%We want to identify zero days in other applications using a systematic approach – by analyzing potential cases where NC can occur.
\fi
\begin{comment}
\begin{enumerate}
\item Create the following:
	% Note that creating `post-checkout' is deferred.

    \parbox{\linewidth}{
    \dirtree{%
     .1 A/\DTcomment{(defer creating `post-checkout')}.
     .2 file1.
     .2 file2.
    }
    }

\item To create `a' (symlink to .git/hooks/), delete `A/' and its contents. This happens since file system is case insensitive.

\item Create `A/post-checkout'. Here, `A' creates a collision with `a`. So instead the following is created: `a/post-checkout`. The operating system further resolves the path into `.git/hooks/post-checkout'.

\item After completing the clone and checkout, git executes `.git/hooks/post-checkout' without realizing that it got created due to a malicious checkout.  Consider the repository structure in \autoref{fig:git-example}. Note that all files (except .git/) are staged and committed in the same order as presented.

\end{enumerate}
\end{comment}

\begin{comment}
This enables the adversary to trick \git\ into running the adversary-controlled script 'post-checkout' after the files are committed.
The `post-checkout' script that \git\ executes is actually part of the repository which was maliciously created. This is because '.git/hooks/' should never be written to by \git; only read from. The .git/hooks/ directory strictly represents scripts installed by the local user for taking certain actions like running code lint, running tests, etc.  \trent{still unclear when/if post-checkout would be installed normally.}

The root cause of the above CVE is the collision between the symbolic link (`a') and the directory (`A'). \git\ fails to recognize that creating `A/post-checkout' is resolved as `a/post-checkout' by the operating system.
\end{comment}

\begin{comment}
While vulnerabilities due to name collisions may appear to be similar to squat vulnerabilities~\cite{mitre-cwe} (CWE-283) on the surface, name collisions provide additionally ways that the victim may be directed to an adversary-controlled file.  In traditional resource squatting scenario, an adversary predicts the name of a file that will be created by a victim and creates that file before the victim does, giving the adversary access to a file that the victim uses to leak or modify victim data.  This attack is possible because the adversary has write access to the directory where the victim will create the file (e.g., {\tt /tmp}).  Name collisions expand the attack surface for such vulnerabilities because the victim willingly uses adversary-defined names to create the colliding files itself, so the adversary does not require write access to the directory where the file will be created to launch attacks.  In addition, the colliding file name may differ from the 

However, we find that name collisions create new ways to lure victims into scenarios that may exploit vulnerabilities and few defenses for these scenarios are currently available.  
% Later: Researchers have studied defenses to prevent aliasing attacks extensively~\cite{nameguard,dean-hu,tsafrir,safeopen,jigsaw14usenix}.  On the other hand, vulnerabilities due to collisions have not been studied in depth.  
%In this paper, we focus primarily on studying how vulnerabilities can emerge when files and directories from case-sensitive file systems are moved/copied to case-insensitive file systems.
% However, motivated by recent vulnerabilities and the increased potential for collisions, we propose to study the security impact of name collisions to determine how such collisions may cause vulnerabilities and assess systems to detect vulnerable scenarios.

Researchers have long known that programs are vulnerable when using symbolic  links, especially those that exploit time-of-check-to-time-of-use (TOCTTOU) vulnerabilities~\cite{mcphee74,bishop-dilger,cai09oakland,chari11ndss,sting12usenix}.  By design, symbolic links provide adversaries with a means to create alternative names for the same resource.  If the adversary has the privilege to write to a directory used by the victim in name resolution or provide a malicious input to the victim used to create a name, the adversary can lure the victim to use an adversary-defined symbolic link to redirect the victim to the aliased file.  
\end{comment}

\begin{comment}
First, if an adversary has write permission to a directory used in name resolution, the adversary may plant an aliasing resource (i.e., symbolic link, hard link, or bind mount) in the directory of a name the victim will use in resolution.  Adversaries may use aliasing to launch two kinds of attacks.  First, an adversary can direct the victim to a file system resource  controlled by the adversary by creating the aliasing resources before the victim, called a {\em file squatting attack}.  Second, an adversary can use the aliasing resource to direct the victim to a file that the adversary is not authorized to access to modify or leak its contents illicitly, called a {\em link traversal attack}. 
\end{comment}


\iffalse
% Explanation
Typically, git allows the creation of file system objects using symlinks. This is intended behavior when the target is within the repository (with the exception of .git/). Moreover, git also sets permissions on the newly created objects.
In the above example, git fails to update its internal state to mark `A' as deleted.  \trent{Why is that important?}

However, {\tt .git/hooks/} is a special folder containing scripts. Scripts with executable permissions are considered active and are executed by git when certain events occur. The script names represent the events (e.g.,  post-checkout refers to the event of completing the checkout phase).  For a successful attack, the following order of events needs to occur: case collision $\rightarrow$ symlink traversal $\rightarrow$ code execution.
To prevent this attack, it is sufficient to block the ``case collision'' between the symlink ('a') and directory name ('A'). \footnote{Git's official fix is to correctly update its internal state to mark the deletion of `A'.}



\trent{The detail below is better suited to the case study.  What's in the case study is more appropriate here.  Summarize 1-4 steps here and include detailed sequence in the case study.  The Analysis from the case study (first two paragraphs max) should appear here as well, but in the same section. }
Consider the repository structure for {\tt repo} in \autoref{fig:git-example}. First, the .git directory contains information needed by \git\ for revision control, some configuration files and certain local scripts. This is explained in more detail in \autoref{sec:git-analysis}.  The directory 'A', its files, and the symbolic link 'a' are part of a repository crafted to launch an attack on \git.

\begin{figure}[h]
\dirtree{%
 .1 repo/.
 .2 .git/.
 .3 hooks/\DTcomment{(local scripts)}.
 .3 objects.
 .3 (redacted).
 .2 A/.
 .3 file1.
 .3 file2.
 .3 post-checkout\DTcomment{(executable script)}.
 .2 a\DTcomment{(symlink to .git/hooks/)}.
}

\caption{Example of the operations resulting from a {\tt clone} of a maliciously crafted file system designed to exploit CVE-2021-21300.}
\label{fig:git-example}
\end{figure}

The above directory structure works correctly when cloned on a case-sensitive file system.  However, when cloned on a case-insensitive file system, the presence of `a' (small) and `A' (capital) creates a collision. Moreover, note that `a' is a symbolic link pointing to the .git/hooks/.

Generally, \git\ identifies that a case-based collision has occurred and places only one of the colliding entries in the directory. However, under certain situations \git\ fails to identify the collision and ends up creating files from `A/' by traversing the symbolic link `a/'.

To understand these special situations, let us look at how \git\ stores the versioning information. Typically all revisions of all files are located inside the .git/objects/ directory. However, storing revisions of binaries can incur a large size overhead. For such cases \git\ supports retrieving the binaries using special backends. These backends are simply external programs that fetch the requested files from a remote server and give it to \git. Note that the user can mark any file inside the repository to be handled by these special backends.

Now, say that the repository creator (the adversary) has marked `post-checkout' file to be retrieved using one of these special backends. This means that `post-checkout' files need to be downloaded from a remote location. When a benign user clones the above repository on a case-insensitive file system (e.g., NTFS), \git\ does the following:

\begin{enumerate}
\item Create the following. Ask the special backend to download `post-checkout' in background.
	% Note that creating `post-checkout' is deferred.

    \parbox{\linewidth}{
    \dirtree{%
     .1 repo/.
     .2 .git/\DTcomment{(redacted)}.
     .2 A/\DTcomment{(defer creating `post-checkout')}.
     .3 file1.
     .3 file2.
    }
    }

\item In order to create `a' (symlink to .git/hooks/), \git\ deletes `A/' and its contents because `a` collides with `A'.

    \parbox{\linewidth}{
    \dirtree{%
     .1 repo/.
     .2 .git/\DTcomment{(redacted)}.
     .2 a/\DTcomment{(symlink to .git/hooks/)}.
    }
    }

\item Create `A/post-checkout'. Here, `A' resolves to `a` (collision) since we're using a case-insensitive file system. The operating system further resolves the path to `.git/hooks/post-checkout'.

\item On completing the above, \git\ triggers an internal event called post-checkout. When this event is triggered, \git\ is programmed to executes the script named `.git/hooks/post-checkout' if it is present and marked as executable.

\end{enumerate}

The `post-checkout' script that \git\ executes is actually part of the repository which was maliciously created. This is because .git/hooks/ should never be written to by \git; only read from. The .git/hooks/ directory strictly represents scripts installed by the local user for taking certain actions like running code lint, running tests, etc.  \trent{still unclear when/if post-checkout would be installed normally.}

The root cause of the above CVE is the collision between the symbolic link (`a') and the directory (`A'). \git\ fails to recognize that creating `A/post-checkout' is resolved as `a/post-checkout' by the operating system.
\fi

\begin{comment}

\section{Security Implications of Collisions}
% ---------------
Several security properties can be violated when collisions occur. These properties are:

\begin{description}
\item[Secrecy] Leaking confidential data. See \autoref{subsec:backup}, \autoref{tab:tooling} -- f4.

\item[Integrity] Corrupting system data. See \autoref{subsec:git}, \autoref{subsec:dpkg}, \autoref{tab:tooling} -- f1, f3, d1.

\item[Privilege Escalation] Gain extra permissions such as read, write, execute, or a combination of these. See \autoref{subsec:httpd}, \autoref{tab:tooling} -- f2, d2.


\item[Denial of Service] Collisions can cause invoked utilities to hang indefinitely. See \todo{FIXME FIXME FIXME}.
\end{description}

In the remainder of this section, we detail our assumed threat model under which the above may occur, describe the operations involved in causing name collisions, and discuss the attack surface for name collisions and the limitations of current defenses.
\end{comment}

==> TODO.tex <==
\section*{Pending}
% ---------------
Rest of the paper:

\begin{itemize}

\item Background
\begin{itemize}
	\item Explain: Case preserving, case normalizing, case insensitive
	\item File squatting is an orthogonal issue. It's one of the ways to get a collision.

When copying files to a case-insensitive FS, the presence of a colliding case can result in squat-like behavior. However, unlike traditional file squatting there need not be another adversary created (squatted) file.

When using a case-insensitive FS, the program can be led to self-squat (squat itself) if the file names come from an untrusted source. Example: remote git repo., archives like tar, files in /tmp, etc.

	\item Policies: named-based, content-based, target-based
	\item Underlying issues: name OR target may be wrong?
\end{itemize}

\item Case Collision
\begin{itemize}
	\item Define it % add Venn diagram
	\item Our invariants % (see A9 and A20)
	\item Shadowing from implicit ordering % (see A50)
\end{itemize}

\item Encoding Collision
\begin{itemize}
	\item Types: conversion and OS normalization % (see A63)
	\item Why we only care about conversion? % (ex. introduccion $\rightarrow$ introducci?n)
	\item Explain: why our monitoring catches these too
\end{itemize}

\item Case Studies
\begin{itemize}
    % Samba scenario: see A48, A50
    \item Past Git CVEs. Does our monitoring catch these?
    \item Other apps affected by NC % cp (see A18)
    \item Which experiments to run?
\end{itemize}

\item Monitoring
\begin{itemize}
	\item Templates % (see PPT and A55)
	\item Algorithm
	\item False positives % (see A62)
\end{itemize}

\item Defense % (see A2, A3, A5, A12)
\begin{itemize}
	\item How existing programs handle this? % see rclone doc: Dropbox
	\item Do programs adhere to our guidelines? % i.e. our version of safe copy
	\item Implications of naming, checking at creation, checking at use etc. What are the pros and cons these approaches?
\end{itemize}

\end{itemize}

* Maliciously crafted names, I get additional perms./authorized access.
* What are the unauthorized access in a repo.?
	* In git, it's the .git directory
	* For httpd, it's the .htacess and perms on folders. The same user's directory can be make public due to a collision.

Characterize cleanly and neatly. Detect additional perms. become available. Identify adversarial FS objects/entities.
1. Modify stuff outside the repo.
2. Who gets perms to the repos
3. Modify code that's gets executed

Flow of paper —
* First, basic scenario. What are the basic perms?
* Second, go over the consistency table. What's the extra perm table?
* Third, apps like git, httpd etc.

Research Questions —
* How common are case collisions (CC)?
* Do programs already implement some defenses against CC?
* How to catch them with low false positive rates?

* Intro. about 5 paragraphs. Balance the last three paragraphs to focus on selling the idea (the insight or system design or evaluation).
	* about the area: files are open by name etc. (be crisp)
	* Problem statement/paragraph. Various security problems occur, etc. etc. Show the figure from outline. We're going to focus on 2nd one or this subset.
	* Related work. Most stuff is related to aliasing. For collisions, its mostly programmers randomly doing stuff
	* Insight paragraph. We need to understand these vulnerabilities in a systematic way. We can discover when there are potentially hazardous situations. We can at least detect and attempt to detect collisions without rewriting their code (with safety properties). We can detect these with signatures with sufficient accuracy.
	* System design paragraph
	* Evaluation paragraph

Meta questions —
* What do we want to talk about?
* Why don't we like the world we live in?
* Why haven't people already solved this already?
* Give some foreshadowing, did you so something about it to solve it. Give an highlight. Some evidence that when you read the paper, there are going to results that you care about.

Section 3: (show people what our reality is)
(list all stories in bullet points)
* Explain why this is a non-trivial challenge and its not going away anytime soon.
* My other motivation — ext4 added support for per-directory case insensitivity
	* Why does not using a case insensitive file systems? And just saying don't do it isn't good enough — avoid this.
	* Even on macOS: things need to work on both case and icase systems.
	* Names in some file systems just cannot be encoded in other file systems. Things on a single file system can go wrong. ext4 is a good example
	* Sell → "There is no consistency in how name resolution is done." List all ways that things go wrong. Then we explain the most common ones we see.
	* What about Turkish to another Locale?
	* We should go though anecdotes: Why you should care about case insensitivity? Why it's something that can happen to you? Why programs are not ready for this? (Answers: Why do we still have these issues?)

Notes —
* We should not call out any heuristic. This is for defense paper. Look at the Cai TOUCTOU paper.
* For paper
	* Document inconsistencies
	* Why it's problematic in practice?
	* We need to demonstrate this using something concrete: ex. diff/patch or another program.
	* We need to show them — Why should they care from a security standpoint?
* Can we never find a correct solution? — Oakland 2009, TOCTOU attack by Cai and Johnson
	* What are the fixes that people have been doing?
	* Any structure to the fixes?
* CITE: Linus on case insensitive file systems
* We have different standards for encodings. It's not a solvable problem. So we need to address it.
* Cloning Linux kernel on macOS doesn't work.
* Trent: If you can add a summary of the research questions and the analysis approach(es) for answering those questions to the outline, I think that would be a good start.
* We don't need many more examples — since it's an existence proof.
* TOOL: What and when can we detect these problems with out testing?
* We may not have a rich collection of CVEs is because it's an understudied field.
* Add results and related work
* Speculate on how to fix the link issue — if we have pages remaining

Evaluation —
* Are there any metrics from our tool? Any objective numbers?
* What are the false positive rates? Don't over explain implementation details — like missing hard link checks. (Avoid airing your own dirty laundry. Just show the final suit.)
* List of quantitative or qualitative metrics. What are things that people will realistically ask?
* The table shows a list of attack vectors. We can assign a percentage to the programs showing its attack surface.

Defense (future work) —
* Define the highest bar of security
* Only allow movement to looser file systems — ASCII to UTF-8. Constraints on the system.
* The OS does not know the application's intent
	* Insight: create time / use time — detect multiple names
* Developer-side/program-side changes. Races that can occur. Make a version of safe-open?
* safecopy library: systematically reason about copy (with consistency)


==> rebuttal.tex <==
\section{Rebuttal Points}

\subsection{Our Contributions}
To the best of our knowledge, ours is the first work studying how case interplays cause vulnerabilities due to name collisions.  We show that utilities and applications do not recognize unsafe use of icase filesystems, leading to exploitable operations. This paper demonstrates the potential security implications of the collision problem, focusing on Linux (see \#4 Testing), thereby motivating both more and broader (e.g., other OS) investigations. 

\subsection{WSL}
WSL exposes Windows files via mount points inside Linux. For example, the user's directories on Windows can be accessed from {\tt /mnt/c/Users/foo}. Since Windows uses a case-insensitive filesystem, all name resolutions inside {\tt /mnt/c} are case-insensitive. Hence, copying or moving files/directories from within Linux to Windows are susceptible to name collisions.

For e.g., running {\tt tar -xvf data.tar.gz -C /mnt/c/Users/foo} will result in a name collision if {\tt data.tar.gz} contains files differing only in case.

\subsection{Ext4 Features}
% https://lwn.net/Articles/784041/
% https://www.kernel.org/doc/html/v5.2/admin-guide/ext4.html

Linux kernel version 5.2 added support for per-directory case-insensitivity to ext4\cite{ext4-support}. For case-insensitive directories, the filesystem is case-preserving in nature. To use this feature, \emph{casefold} option needs to be used when creating the filesystem. For e.g., {\tt mkfs -t ext4 -O casefold /dev/sda}. The newly created filesystem supports mixing case-sensitive and case-insensitive directories on the same filesystem.

Setting the {\tt +F} inode attribute on an empty directory makes it case-insensitive. For e.g., {\tt mkdir foo; chattr +F foo}. Note that case-insensitive directories can contain case-sensitive directories. This means that for a given path, {\tt /foo/bar/bin/baz}, any of {\tt foo}, {\tt bar} and {\tt bin} can either be case-sensitive or case-insensitive.

% discuss "strict" mode? -- it forces filenames to be valid UTF-8 strings

\subsection{Threat Model}

\begin{description}
\item[General] Only happens when moving from case to icase (reviewer B concern) – FALSE. Differences in icase filesystem can also lead to this ex. ext4 icase to ZFS icase. The idea that many-to-one mapping creates the problem.

\item[Define user] end-user, developer, package maintainer, release shepherd etc.

\item[dpkg] run arbitrary code in post-install scripts? Even easier to hide from user because list of files isn’t shown (Reviewer E)

\item[rsync] is it really an alias issue?  Errors in collision defense enable alias exploit

\item[/var/mail] scenario: users not part of the “mail” group cannot create files inside it.

\item[icase tmpfs] Add case-insensitive support for tmpfs (May 2021)\cite{lwn-case-tmpfs}

\end{description}

\subsection{Ethical Disclosure}
We have reported vulnerabilities to dpkg and rsync maintainers. In both cases, they have chosen to update their package documentation to warn end user communities not to use these programs where targets may be case-insensitive (icase) directories.  During discussions with the dpkg maintainers, we analyzed 74,688 packages and found 12,237 filenames from those packages would collide if an icase filesystem were used, breaking these packages.  For rsync, the maintainer replied that rsync is written for case-honoring systems, and this [rsyncing from case to icase] is something that the user shouldn’t do.  At present, rsync does not even account for differences across multiple case-honoring systems, which can also lead to similar collisions (e.g., Kelvin sign, see §2.3).

We are continuing discussions with the maintainers to show that the problem is increasing in significance and that the onus for addressing the problem should not be on the end user. Based on our experiences with these maintainers, we will report to other maintainers soon (e.g., Apache). Before publicly disclosing the vulnerabilities, we will give the maintainers at least 90 days to implement any remedial measures.

